Differentiable Segmentation of Sequences

Segmented models are widely used to describe non-stationary sequential data with discrete change points. Their estimation usually requires solving a mixed discrete-continuous optimization problem, where the segmentation is the discrete part and all other model parameters are continuous. A number of estimation algorithms have been developed that are highly specialized for their specific model assumptions. The dependence on non-standard algorithms makes it hard to integrate segmented models in state-of-the-art deep learning architectures that critically depend on gradient-based optimization techniques. In this work, we formulate a relaxed variant of segmented models that enables joint estimation of all model parameters, including the segmentation, with gradient descent. We build on recent advances in learning continuous warping functions and propose a novel family of warping functions based on the two-sided power (TSP) distribution. TSP-based warping functions are differentiable, have simple closed-form expressions, and can represent segmentation functions exactly. Our formulation includes the important class of segmented generalized linear models as a special case, which makes it highly versatile. We use our approach to model the spread of COVID-19 with Poisson regression, apply it on a change point detection task, and learn classification models with concept drift. The experiments show that our approach effectively learns all these tasks with standard algorithms for gradient descent.

==> ms-gnuplottex-fig1.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(5740.00,1420.00)%
    \gplgaddtomacro\gplbacktext{%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(5694,1246){\makebox(0,0)[l]{\strut{}\scriptsize{$\gamma_1$}}}%
      \csname LTb\endcsname%%
      \put(5694,1042){\makebox(0,0)[l]{\strut{}\scriptsize{$\gamma_2$}}}%
      \csname LTb\endcsname%%
      \put(5694,838){\makebox(0,0)[l]{\strut{}\scriptsize{$\gamma_3$}}}%
      \csname LTb\endcsname%%
      \put(5694,634){\makebox(0,0)[l]{\strut{}\scriptsize{$\zeta$}}}%
      \csname LTb\endcsname%%
      \put(462,403){\makebox(0,0)[r]{\strut{}\scriptsize{1}}}%
      \csname LTb\endcsname%%
      \put(462,887){\makebox(0,0)[r]{\strut{}\scriptsize{2}}}%
      \csname LTb\endcsname%%
      \put(462,1371){\makebox(0,0)[r]{\strut{}\scriptsize{3}}}%
      \csname LTb\endcsname%%
      \put(574,151){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(976,151){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(1377,151){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(1779,151){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(2181,151){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(2583,151){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(2984,151){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(3386,151){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(3788,151){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(4189,151){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(4591,151){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(4703,403){\makebox(0,0)[l]{\strut{}\scriptsize{0}}}%
      \csname LTb\endcsname%%
      \put(4703,887){\makebox(0,0)[l]{\strut{}\scriptsize{0.5}}}%
      \csname LTb\endcsname%%
      \put(4703,1371){\makebox(0,0)[l]{\strut{}\scriptsize{1}}}%
      \csname LTb\endcsname%%
      \put(172,249){\makebox(0,0)[r]{\strut{}\scriptsize{$t=$}}}%
      \csname LTb\endcsname%%
      \put(172,89){\makebox(0,0)[r]{\strut{}\scriptsize{$u_t=$}}}%
      \csname LTb\endcsname%%
      \put(574,249){\makebox(0,0){\strut{}\scriptsize{1}}}%
      \csname LTb\endcsname%%
      \put(976,249){\makebox(0,0){\strut{}\scriptsize{2}}}%
      \csname LTb\endcsname%%
      \put(1377,249){\makebox(0,0){\strut{}\scriptsize{3}}}%
      \csname LTb\endcsname%%
      \put(1779,249){\makebox(0,0){\strut{}\scriptsize{4}}}%
      \csname LTb\endcsname%%
      \put(2181,249){\makebox(0,0){\strut{}\scriptsize{5}}}%
      \csname LTb\endcsname%%
      \put(2583,249){\makebox(0,0){\strut{}\scriptsize{6}}}%
      \csname LTb\endcsname%%
      \put(2984,249){\makebox(0,0){\strut{}\scriptsize{7}}}%
      \csname LTb\endcsname%%
      \put(3386,249){\makebox(0,0){\strut{}\scriptsize{8}}}%
      \csname LTb\endcsname%%
      \put(3788,249){\makebox(0,0){\strut{}\scriptsize{9}}}%
      \csname LTb\endcsname%%
      \put(4189,249){\makebox(0,0){\strut{}\scriptsize{10}}}%
      \csname LTb\endcsname%%
      \put(4591,249){\makebox(0,0){\strut{}\scriptsize{11}}}%
      \csname LTb\endcsname%%
      \put(574,89){\makebox(0,0){\strut{}\scriptsize{0  }}}%
      \csname LTb\endcsname%%
      \put(976,89){\makebox(0,0){\strut{}\scriptsize{0.1}}}%
      \csname LTb\endcsname%%
      \put(1377,89){\makebox(0,0){\strut{}\scriptsize{0.2}}}%
      \csname LTb\endcsname%%
      \put(1779,89){\makebox(0,0){\strut{}\scriptsize{0.3}}}%
      \csname LTb\endcsname%%
      \put(2181,89){\makebox(0,0){\strut{}\scriptsize{0.4}}}%
      \csname LTb\endcsname%%
      \put(2583,89){\makebox(0,0){\strut{}\scriptsize{0.5}}}%
      \csname LTb\endcsname%%
      \put(2984,89){\makebox(0,0){\strut{}\scriptsize{0.6}}}%
      \csname LTb\endcsname%%
      \put(3386,89){\makebox(0,0){\strut{}\scriptsize{0.7}}}%
      \csname LTb\endcsname%%
      \put(3788,89){\makebox(0,0){\strut{}\scriptsize{0.8}}}%
      \csname LTb\endcsname%%
      \put(4189,89){\makebox(0,0){\strut{}\scriptsize{0.9}}}%
      \csname LTb\endcsname%%
      \put(4591,89){\makebox(0,0){\strut{}\scriptsize{1  }}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{fig1}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> ms-gnuplottex-fig2.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(7900.00,2860.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(857,1601){\makebox(0,0)[l]{\strut{}\tiny{mode}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(789,2593){\makebox(0,0){\strut{}\small{$\operatorname{TSP}(0.5, 1, 2)$}}}%
      \csname LTb\endcsname%%
      \put(112,1226){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(383,1226){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(654,1226){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(925,1226){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(1196,1226){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(1467,1226){\makebox(0,0){\strut{}}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(356,952){\makebox(0,0)[l]{\strut{}\tiny{width}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(112,225){\makebox(0,0){\strut{}\tiny{0}}}%
      \csname LTb\endcsname%%
      \put(383,225){\makebox(0,0){\strut{}\tiny{0.2}}}%
      \csname LTb\endcsname%%
      \put(654,225){\makebox(0,0){\strut{}\tiny{0.4}}}%
      \csname LTb\endcsname%%
      \put(925,225){\makebox(0,0){\strut{}\tiny{0.6}}}%
      \csname LTb\endcsname%%
      \put(1196,225){\makebox(0,0){\strut{}\tiny{0.8}}}%
      \csname LTb\endcsname%%
      \put(1467,225){\makebox(0,0){\strut{}\tiny{1}}}%
    }%
    \gplgaddtomacro\gplbacktext{%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(2369,2593){\makebox(0,0){\strut{}\small{$\operatorname{TSP}(0.5, 1, 4)$}}}%
      \csname LTb\endcsname%%
      \put(1692,1226){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(1963,1226){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(2234,1226){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(2505,1226){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(2776,1226){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(3047,1226){\makebox(0,0){\strut{}}}%
    }%
    \gplgaddtomacro\gplbacktext{%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1692,225){\makebox(0,0){\strut{}\tiny{0}}}%
      \csname LTb\endcsname%%
      \put(1963,225){\makebox(0,0){\strut{}\tiny{0.2}}}%
      \csname LTb\endcsname%%
      \put(2234,225){\makebox(0,0){\strut{}\tiny{0.4}}}%
      \csname LTb\endcsname%%
      \put(2505,225){\makebox(0,0){\strut{}\tiny{0.6}}}%
      \csname LTb\endcsname%%
      \put(2776,225){\makebox(0,0){\strut{}\tiny{0.8}}}%
      \csname LTb\endcsname%%
      \put(3047,225){\makebox(0,0){\strut{}\tiny{1}}}%
    }%
    \gplgaddtomacro\gplbacktext{%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(3949,2593){\makebox(0,0){\strut{}\small{$\operatorname{TSP}(0.5, 0.5, 4)$}}}%
      \csname LTb\endcsname%%
      \put(3272,1226){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(3543,1226){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(3814,1226){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(4085,1226){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(4356,1226){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(4627,1226){\makebox(0,0){\strut{}}}%
    }%
    \gplgaddtomacro\gplbacktext{%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(3272,225){\makebox(0,0){\strut{}\tiny{0}}}%
      \csname LTb\endcsname%%
      \put(3543,225){\makebox(0,0){\strut{}\tiny{0.2}}}%
      \csname LTb\endcsname%%
      \put(3814,225){\makebox(0,0){\strut{}\tiny{0.4}}}%
      \csname LTb\endcsname%%
      \put(4085,225){\makebox(0,0){\strut{}\tiny{0.6}}}%
      \csname LTb\endcsname%%
      \put(4356,225){\makebox(0,0){\strut{}\tiny{0.8}}}%
      \csname LTb\endcsname%%
      \put(4627,225){\makebox(0,0){\strut{}\tiny{1}}}%
    }%
    \gplgaddtomacro\gplbacktext{%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(5529,2593){\makebox(0,0){\strut{}\small{$\operatorname{TSP}(0.7, 0.5, 4)$}}}%
      \csname LTb\endcsname%%
      \put(4852,1226){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(5123,1226){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(5394,1226){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(5665,1226){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(5936,1226){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(6207,1226){\makebox(0,0){\strut{}}}%
    }%
    \gplgaddtomacro\gplbacktext{%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(4852,225){\makebox(0,0){\strut{}\tiny{0}}}%
      \csname LTb\endcsname%%
      \put(5123,225){\makebox(0,0){\strut{}\tiny{0.2}}}%
      \csname LTb\endcsname%%
      \put(5394,225){\makebox(0,0){\strut{}\tiny{0.4}}}%
      \csname LTb\endcsname%%
      \put(5665,225){\makebox(0,0){\strut{}\tiny{0.6}}}%
      \csname LTb\endcsname%%
      \put(5936,225){\makebox(0,0){\strut{}\tiny{0.8}}}%
      \csname LTb\endcsname%%
      \put(6207,225){\makebox(0,0){\strut{}\tiny{1}}}%
    }%
    \gplgaddtomacro\gplbacktext{%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(7109,2593){\makebox(0,0){\strut{}\small{$\operatorname{TSP}(0.9, 0.5, 4)$}}}%
      \csname LTb\endcsname%%
      \put(6432,1226){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(6703,1226){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(6974,1226){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(7245,1226){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(7516,1226){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(7787,1226){\makebox(0,0){\strut{}}}%
    }%
    \gplgaddtomacro\gplbacktext{%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(6432,225){\makebox(0,0){\strut{}\tiny{0}}}%
      \csname LTb\endcsname%%
      \put(6703,225){\makebox(0,0){\strut{}\tiny{0.2}}}%
      \csname LTb\endcsname%%
      \put(6974,225){\makebox(0,0){\strut{}\tiny{0.4}}}%
      \csname LTb\endcsname%%
      \put(7245,225){\makebox(0,0){\strut{}\tiny{0.6}}}%
      \csname LTb\endcsname%%
      \put(7516,225){\makebox(0,0){\strut{}\tiny{0.8}}}%
      \csname LTb\endcsname%%
      \put(7787,225){\makebox(0,0){\strut{}\tiny{1}}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{fig2}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> ms-gnuplottex-fig3.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(7180.00,1780.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(606,356){\makebox(0,0)[r]{\strut{}\tiny{-10000}}}%
      \csname LTb\endcsname%%
      \put(606,497){\makebox(0,0)[r]{\strut{}\tiny{-9000}}}%
      \csname LTb\endcsname%%
      \put(606,637){\makebox(0,0)[r]{\strut{}\tiny{-8000}}}%
      \csname LTb\endcsname%%
      \put(606,778){\makebox(0,0)[r]{\strut{}\tiny{-7000}}}%
      \csname LTb\endcsname%%
      \put(606,918){\makebox(0,0)[r]{\strut{}\tiny{-6000}}}%
      \csname LTb\endcsname%%
      \put(606,1059){\makebox(0,0)[r]{\strut{}\tiny{-5000}}}%
      \csname LTb\endcsname%%
      \put(606,1199){\makebox(0,0)[r]{\strut{}\tiny{-4000}}}%
      \csname LTb\endcsname%%
      \put(606,1340){\makebox(0,0)[r]{\strut{}\tiny{-3000}}}%
      \csname LTb\endcsname%%
      \put(606,1480){\makebox(0,0)[r]{\strut{}\tiny{-2000}}}%
      \csname LTb\endcsname%%
      \put(606,1621){\makebox(0,0)[r]{\strut{}\tiny{-1000}}}%
      \csname LTb\endcsname%%
      \put(606,1761){\makebox(0,0)[r]{\strut{}\tiny{0}}}%
      \csname LTb\endcsname%%
      \put(718,254){\makebox(0,0){\strut{}\tiny{2}}}%
      \csname LTb\endcsname%%
      \put(1077,254){\makebox(0,0){\strut{}\tiny{4}}}%
      \csname LTb\endcsname%%
      \put(1436,254){\makebox(0,0){\strut{}\tiny{8}}}%
      \csname LTb\endcsname%%
      \put(1794,254){\makebox(0,0){\strut{}\tiny{16}}}%
      \csname LTb\endcsname%%
      \put(2153,254){\makebox(0,0){\strut{}\tiny{32}}}%
      \csname LTb\endcsname%%
      \put(2512,254){\makebox(0,0){\strut{}\tiny{64}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1615,50){\makebox(0,0){\strut{}\scriptsize{number of segments $K$}}}%
      \csname LTb\endcsname%%
      \put(1871,986){\makebox(0,0)[r]{\strut{}\tiny{saturated model}}}%
      \csname LTb\endcsname%%
      \put(1871,864){\makebox(0,0)[r]{\strut{}\tiny{Muggeo (2003)}}}%
      \csname LTb\endcsname%%
      \put(1871,742){\makebox(0,0)[r]{\strut{}\tiny{CPAb}}}%
      \csname LTb\endcsname%%
      \put(1871,620){\makebox(0,0)[r]{\strut{}\tiny{NP}}}%
      \csname LTb\endcsname%%
      \put(1871,498){\makebox(0,0)[r]{\strut{}\tiny{TSPb}}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(3478,356){\makebox(0,0)[r]{\strut{}\tiny{0}}}%
      \csname LTb\endcsname%%
      \put(3478,532){\makebox(0,0)[r]{\strut{}\tiny{1000}}}%
      \csname LTb\endcsname%%
      \put(3478,707){\makebox(0,0)[r]{\strut{}\tiny{2000}}}%
      \csname LTb\endcsname%%
      \put(3478,883){\makebox(0,0)[r]{\strut{}\tiny{3000}}}%
      \csname LTb\endcsname%%
      \put(3478,1059){\makebox(0,0)[r]{\strut{}\tiny{4000}}}%
      \csname LTb\endcsname%%
      \put(3478,1234){\makebox(0,0)[r]{\strut{}\tiny{5000}}}%
      \csname LTb\endcsname%%
      \put(3478,1410){\makebox(0,0)[r]{\strut{}\tiny{6000}}}%
      \csname LTb\endcsname%%
      \put(3478,1585){\makebox(0,0)[r]{\strut{}\tiny{7000}}}%
      \csname LTb\endcsname%%
      \put(3478,1761){\makebox(0,0)[r]{\strut{}\tiny{8000}}}%
      \csname LTb\endcsname%%
      \put(3628,204){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}\tiny{Feb 24}}}}%
      \csname LTb\endcsname%%
      \put(3896,204){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}\tiny{Mar 02}}}}%
      \csname LTb\endcsname%%
      \put(4163,204){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}\tiny{Mar 09}}}}%
      \csname LTb\endcsname%%
      \put(4431,204){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}\tiny{Mar 16}}}}%
      \csname LTb\endcsname%%
      \put(4699,204){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}\tiny{Mar 23}}}}%
      \csname LTb\endcsname%%
      \put(4966,204){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}\tiny{Mar 30}}}}%
      \csname LTb\endcsname%%
      \put(5234,204){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}\tiny{Apr 06}}}}%
      \csname LTb\endcsname%%
      \put(5501,204){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}\tiny{Apr 13}}}}%
      \csname LTb\endcsname%%
      \put(5769,204){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}\tiny{Apr 20}}}}%
      \csname LTb\endcsname%%
      \put(6037,204){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}\tiny{Apr 27}}}}%
      \csname LTb\endcsname%%
      \put(6304,204){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}\tiny{May 04}}}}%
      \csname LTb\endcsname%%
      \put(6572,204){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}\tiny{May 11}}}}%
      \csname LTb\endcsname%%
      \put(6839,204){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}\tiny{May 18}}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(3012,1058){\rotatebox{-270}{\makebox(0,0){\strut{}\scriptsize{new cases}}}}%
      \csname LTb\endcsname%%
      \put(6466,1619){\makebox(0,0)[r]{\strut{}\tiny{reported}}}%
      \csname LTb\endcsname%%
      \put(6466,1497){\makebox(0,0)[r]{\strut{}\tiny{prediction}}}%
      \csname LTb\endcsname%%
      \put(6466,1375){\makebox(0,0)[r]{\strut{}\tiny{average dow}}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{fig3}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> ms-gnuplottex-fig4.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(7180.00,1060.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(112,106){\makebox(0,0)[r]{\strut{}\tiny{0}}}%
      \csname LTb\endcsname%%
      \put(112,291){\makebox(0,0)[r]{\strut{}\tiny{5}}}%
      \csname LTb\endcsname%%
      \put(112,477){\makebox(0,0)[r]{\strut{}\tiny{10}}}%
      \csname LTb\endcsname%%
      \put(112,662){\makebox(0,0)[r]{\strut{}\tiny{15}}}%
      \csname LTb\endcsname%%
      \put(112,847){\makebox(0,0)[r]{\strut{}\tiny{20}}}%
      \csname LTb\endcsname%%
      \put(224,4){\makebox(0,0){\strut{}\tiny{0}}}%
      \csname LTb\endcsname%%
      \put(538,4){\makebox(0,0){\strut{}\tiny{100}}}%
      \csname LTb\endcsname%%
      \put(852,4){\makebox(0,0){\strut{}\tiny{200}}}%
      \csname LTb\endcsname%%
      \put(1166,4){\makebox(0,0){\strut{}\tiny{300}}}%
      \csname LTb\endcsname%%
      \put(1480,4){\makebox(0,0){\strut{}\tiny{400}}}%
      \csname LTb\endcsname%%
      \put(1795,4){\makebox(0,0){\strut{}\tiny{500}}}%
      \csname LTb\endcsname%%
      \put(2109,4){\makebox(0,0){\strut{}\tiny{600}}}%
      \csname LTb\endcsname%%
      \put(2423,4){\makebox(0,0){\strut{}\tiny{700}}}%
      \csname LTb\endcsname%%
      \put(2737,4){\makebox(0,0){\strut{}\tiny{800}}}%
      \csname LTb\endcsname%%
      \put(3051,4){\makebox(0,0){\strut{}\tiny{900}}}%
      \csname LTb\endcsname%%
      \put(3365,4){\makebox(0,0){\strut{}\tiny{1000}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1794,1030){\makebox(0,0){\strut{}\tiny{random sequence (scenario 1)}}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(3702,106){\makebox(0,0)[r]{\strut{}\tiny{0}}}%
      \csname LTb\endcsname%%
      \put(3702,254){\makebox(0,0)[r]{\strut{}\tiny{20}}}%
      \csname LTb\endcsname%%
      \put(3702,402){\makebox(0,0)[r]{\strut{}\tiny{40}}}%
      \csname LTb\endcsname%%
      \put(3702,551){\makebox(0,0)[r]{\strut{}\tiny{60}}}%
      \csname LTb\endcsname%%
      \put(3702,699){\makebox(0,0)[r]{\strut{}\tiny{80}}}%
      \csname LTb\endcsname%%
      \put(3702,847){\makebox(0,0)[r]{\strut{}\tiny{100}}}%
      \csname LTb\endcsname%%
      \put(3814,4){\makebox(0,0){\strut{}\tiny{0}}}%
      \csname LTb\endcsname%%
      \put(4128,4){\makebox(0,0){\strut{}\tiny{100}}}%
      \csname LTb\endcsname%%
      \put(4442,4){\makebox(0,0){\strut{}\tiny{200}}}%
      \csname LTb\endcsname%%
      \put(4756,4){\makebox(0,0){\strut{}\tiny{300}}}%
      \csname LTb\endcsname%%
      \put(5070,4){\makebox(0,0){\strut{}\tiny{400}}}%
      \csname LTb\endcsname%%
      \put(5385,4){\makebox(0,0){\strut{}\tiny{500}}}%
      \csname LTb\endcsname%%
      \put(5699,4){\makebox(0,0){\strut{}\tiny{600}}}%
      \csname LTb\endcsname%%
      \put(6013,4){\makebox(0,0){\strut{}\tiny{700}}}%
      \csname LTb\endcsname%%
      \put(6327,4){\makebox(0,0){\strut{}\tiny{800}}}%
      \csname LTb\endcsname%%
      \put(6641,4){\makebox(0,0){\strut{}\tiny{900}}}%
      \csname LTb\endcsname%%
      \put(6955,4){\makebox(0,0){\strut{}\tiny{1000}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(5384,1030){\makebox(0,0){\strut{}\tiny{TSPb detection frequencies over 500 random sequences}}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{fig4}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> ms-gnuplottex-fig5.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(7180.00,1560.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(606,312){\makebox(0,0)[r]{\strut{}\tiny{0.5}}}%
      \csname LTb\endcsname%%
      \put(606,585){\makebox(0,0)[r]{\strut{}\tiny{0.6}}}%
      \csname LTb\endcsname%%
      \put(606,857){\makebox(0,0)[r]{\strut{}\tiny{0.7}}}%
      \csname LTb\endcsname%%
      \put(606,1130){\makebox(0,0)[r]{\strut{}\tiny{0.8}}}%
      \csname LTb\endcsname%%
      \put(606,1403){\makebox(0,0)[r]{\strut{}\tiny{0.9}}}%
      \csname LTb\endcsname%%
      \put(718,210){\makebox(0,0){\strut{}\tiny{2}}}%
      \csname LTb\endcsname%%
      \put(897,210){\makebox(0,0){\strut{}\tiny{4}}}%
      \csname LTb\endcsname%%
      \put(1077,210){\makebox(0,0){\strut{}\tiny{8}}}%
      \csname LTb\endcsname%%
      \put(1256,210){\makebox(0,0){\strut{}\tiny{16}}}%
      \csname LTb\endcsname%%
      \put(1435,210){\makebox(0,0){\strut{}\tiny{32}}}%
      \csname LTb\endcsname%%
      \put(1615,210){\makebox(0,0){\strut{}\tiny{64}}}%
      \csname LTb\endcsname%%
      \put(1794,210){\makebox(0,0){\strut{}\tiny{128}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(308,857){\rotatebox{-270}{\makebox(0,0){\strut{}\scriptsize{accuracy}}}}%
      \csname LTb\endcsname%%
      \put(1256,6){\makebox(0,0){\strut{}\scriptsize{$K$}}}%
      \csname LTb\endcsname%%
      \put(1256,1556){\makebox(0,0){\strut{}\scriptsize{incremental}}}%
      \csname LTb\endcsname%%
      \put(1247,1261){\makebox(0,0)[l]{\strut{}\tiny{LB}}}%
      \csname LTb\endcsname%%
      \put(1247,1139){\makebox(0,0)[l]{\strut{}\tiny{ARF}}}%
      \csname LTb\endcsname%%
      \put(1247,1017){\makebox(0,0)[l]{\strut{}\tiny{TSPb}}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(1862,312){\makebox(0,0)[r]{\strut{}}}%
      \csname LTb\endcsname%%
      \put(1862,585){\makebox(0,0)[r]{\strut{}}}%
      \csname LTb\endcsname%%
      \put(1862,857){\makebox(0,0)[r]{\strut{}}}%
      \csname LTb\endcsname%%
      \put(1862,1130){\makebox(0,0)[r]{\strut{}}}%
      \csname LTb\endcsname%%
      \put(1862,1403){\makebox(0,0)[r]{\strut{}}}%
      \csname LTb\endcsname%%
      \put(1974,210){\makebox(0,0){\strut{}\tiny{2}}}%
      \csname LTb\endcsname%%
      \put(2154,210){\makebox(0,0){\strut{}\tiny{4}}}%
      \csname LTb\endcsname%%
      \put(2333,210){\makebox(0,0){\strut{}\tiny{8}}}%
      \csname LTb\endcsname%%
      \put(2513,210){\makebox(0,0){\strut{}\tiny{16}}}%
      \csname LTb\endcsname%%
      \put(2692,210){\makebox(0,0){\strut{}\tiny{32}}}%
      \csname LTb\endcsname%%
      \put(2872,210){\makebox(0,0){\strut{}\tiny{64}}}%
      \csname LTb\endcsname%%
      \put(3051,210){\makebox(0,0){\strut{}\tiny{128}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(2512,6){\makebox(0,0){\strut{}\scriptsize{$K$}}}%
      \csname LTb\endcsname%%
      \put(2512,1556){\makebox(0,0){\strut{}\scriptsize{abrupt}}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(3119,312){\makebox(0,0)[r]{\strut{}}}%
      \csname LTb\endcsname%%
      \put(3119,585){\makebox(0,0)[r]{\strut{}}}%
      \csname LTb\endcsname%%
      \put(3119,857){\makebox(0,0)[r]{\strut{}}}%
      \csname LTb\endcsname%%
      \put(3119,1130){\makebox(0,0)[r]{\strut{}}}%
      \csname LTb\endcsname%%
      \put(3119,1403){\makebox(0,0)[r]{\strut{}}}%
      \csname LTb\endcsname%%
      \put(3231,210){\makebox(0,0){\strut{}\tiny{2}}}%
      \csname LTb\endcsname%%
      \put(3410,210){\makebox(0,0){\strut{}\tiny{4}}}%
      \csname LTb\endcsname%%
      \put(3590,210){\makebox(0,0){\strut{}\tiny{8}}}%
      \csname LTb\endcsname%%
      \put(3769,210){\makebox(0,0){\strut{}\tiny{16}}}%
      \csname LTb\endcsname%%
      \put(3948,210){\makebox(0,0){\strut{}\tiny{32}}}%
      \csname LTb\endcsname%%
      \put(4128,210){\makebox(0,0){\strut{}\tiny{64}}}%
      \csname LTb\endcsname%%
      \put(4307,210){\makebox(0,0){\strut{}\tiny{128}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(3769,6){\makebox(0,0){\strut{}\scriptsize{$K$}}}%
      \csname LTb\endcsname%%
      \put(3769,1556){\makebox(0,0){\strut{}\scriptsize{inc-gradual}}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(4375,312){\makebox(0,0)[r]{\strut{}}}%
      \csname LTb\endcsname%%
      \put(4375,585){\makebox(0,0)[r]{\strut{}}}%
      \csname LTb\endcsname%%
      \put(4375,857){\makebox(0,0)[r]{\strut{}}}%
      \csname LTb\endcsname%%
      \put(4375,1130){\makebox(0,0)[r]{\strut{}}}%
      \csname LTb\endcsname%%
      \put(4375,1403){\makebox(0,0)[r]{\strut{}}}%
      \csname LTb\endcsname%%
      \put(4487,210){\makebox(0,0){\strut{}\tiny{2}}}%
      \csname LTb\endcsname%%
      \put(4666,210){\makebox(0,0){\strut{}\tiny{4}}}%
      \csname LTb\endcsname%%
      \put(4846,210){\makebox(0,0){\strut{}\tiny{8}}}%
      \csname LTb\endcsname%%
      \put(5025,210){\makebox(0,0){\strut{}\tiny{16}}}%
      \csname LTb\endcsname%%
      \put(5204,210){\makebox(0,0){\strut{}\tiny{32}}}%
      \csname LTb\endcsname%%
      \put(5384,210){\makebox(0,0){\strut{}\tiny{64}}}%
      \csname LTb\endcsname%%
      \put(5563,210){\makebox(0,0){\strut{}\tiny{128}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(5025,6){\makebox(0,0){\strut{}\scriptsize{$K$}}}%
      \csname LTb\endcsname%%
      \put(5025,1556){\makebox(0,0){\strut{}\scriptsize{inc-abrupt-reocc}}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(5632,312){\makebox(0,0)[r]{\strut{}}}%
      \csname LTb\endcsname%%
      \put(5632,585){\makebox(0,0)[r]{\strut{}}}%
      \csname LTb\endcsname%%
      \put(5632,857){\makebox(0,0)[r]{\strut{}}}%
      \csname LTb\endcsname%%
      \put(5632,1130){\makebox(0,0)[r]{\strut{}}}%
      \csname LTb\endcsname%%
      \put(5632,1403){\makebox(0,0)[r]{\strut{}}}%
      \csname LTb\endcsname%%
      \put(5744,210){\makebox(0,0){\strut{}\tiny{2}}}%
      \csname LTb\endcsname%%
      \put(5923,210){\makebox(0,0){\strut{}\tiny{4}}}%
      \csname LTb\endcsname%%
      \put(6103,210){\makebox(0,0){\strut{}\tiny{8}}}%
      \csname LTb\endcsname%%
      \put(6282,210){\makebox(0,0){\strut{}\tiny{16}}}%
      \csname LTb\endcsname%%
      \put(6461,210){\makebox(0,0){\strut{}\tiny{32}}}%
      \csname LTb\endcsname%%
      \put(6641,210){\makebox(0,0){\strut{}\tiny{64}}}%
      \csname LTb\endcsname%%
      \put(6820,210){\makebox(0,0){\strut{}\tiny{128}}}%
      \csname LTb\endcsname%%
      \put(6932,312){\makebox(0,0)[l]{\strut{}\tiny{0.5}}}%
      \csname LTb\endcsname%%
      \put(6932,585){\makebox(0,0)[l]{\strut{}\tiny{0.6}}}%
      \csname LTb\endcsname%%
      \put(6932,857){\makebox(0,0)[l]{\strut{}\tiny{0.7}}}%
      \csname LTb\endcsname%%
      \put(6932,1130){\makebox(0,0)[l]{\strut{}\tiny{0.8}}}%
      \csname LTb\endcsname%%
      \put(6932,1403){\makebox(0,0)[l]{\strut{}\tiny{0.9}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(6282,6){\makebox(0,0){\strut{}\scriptsize{$K$}}}%
      \csname LTb\endcsname%%
      \put(6282,1556){\makebox(0,0){\strut{}\scriptsize{inc-reocc}}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{fig5}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> ms-gnuplottex-fig6.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(7180.00,760.00)%
    \gplgaddtomacro\gplbacktext{%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1794,709){\makebox(0,0){\strut{}\tiny{observed sequence, with true phoneme boundaries}}}%
    }%
    \gplgaddtomacro\gplbacktext{%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(5384,709){\makebox(0,0){\strut{}\tiny{predicted sequence, with true phoneme boundaries}}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{fig6}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> ms-gnuplottex-fig7.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(7180.00,1780.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(606,356){\makebox(0,0)[r]{\strut{}\tiny{-3000}}}%
      \csname LTb\endcsname%%
      \put(606,590){\makebox(0,0)[r]{\strut{}\tiny{-2500}}}%
      \csname LTb\endcsname%%
      \put(606,824){\makebox(0,0)[r]{\strut{}\tiny{-2000}}}%
      \csname LTb\endcsname%%
      \put(606,1059){\makebox(0,0)[r]{\strut{}\tiny{-1500}}}%
      \csname LTb\endcsname%%
      \put(606,1293){\makebox(0,0)[r]{\strut{}\tiny{-1000}}}%
      \csname LTb\endcsname%%
      \put(606,1527){\makebox(0,0)[r]{\strut{}\tiny{-500}}}%
      \csname LTb\endcsname%%
      \put(606,1761){\makebox(0,0)[r]{\strut{}\tiny{0}}}%
      \csname LTb\endcsname%%
      \put(718,254){\makebox(0,0){\strut{}\tiny{1024}}}%
      \csname LTb\endcsname%%
      \put(1316,254){\makebox(0,0){\strut{}\tiny{2048}}}%
      \csname LTb\endcsname%%
      \put(1914,254){\makebox(0,0){\strut{}\tiny{4096}}}%
      \csname LTb\endcsname%%
      \put(2512,254){\makebox(0,0){\strut{}\tiny{8192}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(84,1058){\rotatebox{-270}{\makebox(0,0){\strut{}\scriptsize{log-likelihood}}}}%
      \csname LTb\endcsname%%
      \put(1615,50){\makebox(0,0){\strut{}\scriptsize{TSPb integer epochs}}}%
      \csname LTb\endcsname%%
      \put(1247,742){\makebox(0,0)[l]{\strut{}\tiny{saturated model}}}%
      \csname LTb\endcsname%%
      \put(1247,620){\makebox(0,0)[l]{\strut{}\tiny{Muggeo (2003)}}}%
      \csname LTb\endcsname%%
      \put(1247,498){\makebox(0,0)[l]{\strut{}\tiny{TSPb}}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(2760,356){\makebox(0,0)[r]{\strut{}}}%
      \csname LTb\endcsname%%
      \put(2760,590){\makebox(0,0)[r]{\strut{}}}%
      \csname LTb\endcsname%%
      \put(2760,824){\makebox(0,0)[r]{\strut{}}}%
      \csname LTb\endcsname%%
      \put(2760,1059){\makebox(0,0)[r]{\strut{}}}%
      \csname LTb\endcsname%%
      \put(2760,1293){\makebox(0,0)[r]{\strut{}}}%
      \csname LTb\endcsname%%
      \put(2760,1527){\makebox(0,0)[r]{\strut{}}}%
      \csname LTb\endcsname%%
      \put(2760,1761){\makebox(0,0)[r]{\strut{}}}%
      \csname LTb\endcsname%%
      \put(2872,254){\makebox(0,0){\strut{}\tiny{$\frac{1}{64}$}}}%
      \csname LTb\endcsname%%
      \put(3231,254){\makebox(0,0){\strut{}\tiny{$\frac{1}{32}$}}}%
      \csname LTb\endcsname%%
      \put(3590,254){\makebox(0,0){\strut{}\tiny{$\frac{1}{16}$}}}%
      \csname LTb\endcsname%%
      \put(3948,254){\makebox(0,0){\strut{}\tiny{$\frac{1}{8}$}}}%
      \csname LTb\endcsname%%
      \put(4307,254){\makebox(0,0){\strut{}\tiny{$\frac{1}{4}$}}}%
      \csname LTb\endcsname%%
      \put(4666,254){\makebox(0,0){\strut{}\tiny{$\frac{1}{2}$}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(3769,50){\makebox(0,0){\strut{}\scriptsize{TSPb width $w$}}}%
      \csname LTb\endcsname%%
      \put(3401,742){\makebox(0,0)[l]{\strut{}\tiny{saturated model}}}%
      \csname LTb\endcsname%%
      \put(3401,620){\makebox(0,0)[l]{\strut{}\tiny{Muggeo (2003)}}}%
      \csname LTb\endcsname%%
      \put(3401,498){\makebox(0,0)[l]{\strut{}\tiny{TSPb}}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(4914,356){\makebox(0,0)[r]{\strut{}}}%
      \csname LTb\endcsname%%
      \put(4914,590){\makebox(0,0)[r]{\strut{}}}%
      \csname LTb\endcsname%%
      \put(4914,824){\makebox(0,0)[r]{\strut{}}}%
      \csname LTb\endcsname%%
      \put(4914,1059){\makebox(0,0)[r]{\strut{}}}%
      \csname LTb\endcsname%%
      \put(4914,1293){\makebox(0,0)[r]{\strut{}}}%
      \csname LTb\endcsname%%
      \put(4914,1527){\makebox(0,0)[r]{\strut{}}}%
      \csname LTb\endcsname%%
      \put(4914,1761){\makebox(0,0)[r]{\strut{}}}%
      \csname LTb\endcsname%%
      \put(5026,254){\makebox(0,0){\strut{}\tiny{2}}}%
      \csname LTb\endcsname%%
      \put(5475,254){\makebox(0,0){\strut{}\tiny{4}}}%
      \csname LTb\endcsname%%
      \put(5923,254){\makebox(0,0){\strut{}\tiny{8}}}%
      \csname LTb\endcsname%%
      \put(6372,254){\makebox(0,0){\strut{}\tiny{16}}}%
      \csname LTb\endcsname%%
      \put(6820,254){\makebox(0,0){\strut{}\tiny{32}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(5923,50){\makebox(0,0){\strut{}\scriptsize{TSPb power $n$}}}%
      \csname LTb\endcsname%%
      \put(5555,742){\makebox(0,0)[l]{\strut{}\tiny{saturated model}}}%
      \csname LTb\endcsname%%
      \put(5555,620){\makebox(0,0)[l]{\strut{}\tiny{Muggeo (2003)}}}%
      \csname LTb\endcsname%%
      \put(5555,498){\makebox(0,0)[l]{\strut{}\tiny{TSPb}}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{fig7}}%
    \gplfronttext
  \end{picture}%
\endgroup

